Scalable Application- and User-aware Resource Allocation in Enterprise Networks Using End-host Pacing

Scalable user- and application-aware resource allocation for heterogeneous applications sharing an enterprise network is still an unresolved problem. The main challenges are: (i) How to define user- and application-aware shares of resources? (ii) How to determine an allocation of shares of network resources to applications? (iii) How to allocate the shares per application in heterogeneous networks at scale? In this paper we propose solutions to the three challenges and introduce a system design for enterprise deployment. Defining the necessary resource shares per application is hard, as the intended use case and user's preferences influence the resource demand. Utility functions based on user experience enable a mapping of network resources in terms of throughput and latency budget to a common user-level utility scale. A multi-objective MILP is formulated to solve the throughput- and delay-aware embedding of each utility function for a max-min fairness criteria. The allocation of resources in traditional networks with policing and scheduling cannot distinguish large numbers of classes. We propose a resource allocation system design for enterprise networks based on Software-Defined Networking principles to achieve delay-constrained routing in the network and application pacing at the end-hosts. The system design is evaluated against best effort networks with applications competing for the throughput of a constrained link. The competing applications belong to the five application classes web browsing, file download, remote terminal work, video streaming, and Voice-over-IP. The results show that the proposed methodology improves the minimum and total utility, minimizes packet loss and queuing delay at bottlenecks, establishes fairness in terms of utility between applications, and achieves predictable application performance at high link utilization.

==> content/09_discussion.tex <==
\section{Future Work} \label{sec:discussion}  

The evaluation shows that through centrally-configured flow pacing with accurate intent-specific utility functions the predictability, fairness and utility for most application classes can be improved compared to best effort networks.

This work can be continued in multiple research directions.

\noindent
\textbf{First}, the fairness formulation should be extended to support assignment of priority values to applications.

\noindent
\textbf{Second}, a suitable heuristic has to be developed to find approximate solutions for the fairness problem formulation.

\noindent
\textbf{Third}, it should be evaluated under which conditions and how much end-host pacing can profit from additional in-network QoS measures such as priority queuing or random early drop (RED).

\noindent
\textbf{Forth}, the benefit has to be evaluated for dynamic scenarios and the potential multiplexing gain calculated accordingly.
Specifically for application configurations with longer idle periods between requests.
Static allocation with longer idle periods does not profit from multiplexing gain and the benefit compared to best effort networks decreases.
The benefit in dynamic scenarios could be increased by applying intelligent overbooking according to queuing theory and monitoring of application behavior.

\noindent
\textbf{Fifth}, determine the trade-off between accuracy of the utility function and the resulting utility for the user.
The evaluation shows that when a suitable utility function per application is available data-rate management through pacing results in predictable application performance in terms of utility.
In case the network controller can not determine the precise intent or no utility function is available, fallback policies have to be implemented to approximate the demand of the application through a higher-level intent.
Hence it is important to understand the relationship between inaccurate utility functions and the resulting utility for the user.

\fixme{https://hal-imt.archives-ouvertes.fr/hal-00941783/file/BR11.pdf}

\noindent
\textbf{Sixth}, determine and update utility functions on-demand through status reporting by the applications and user feedback.
Building a complete hierarchy manually of all applications, intents and their utility functions in an enterprise environment is time-consuming.
Instant user feedback combined with monitoring the application KPIs through the agent can help to create or to improve user experience models.
By putting the intent and network parameters, such as pacing rate and delay, in relationship with the KPIs and user experience model, the network controller can autonomously extend or update the hierarchy.
For example, the network controller could monitor the public web-sites requested through the Internet proxy and the resulting page load time.
The network controller could then either create a very specific utility function per web-site or derive a utility function which is valid for most of the requested web-sites.

\noindent
\textbf{Seventh}, build awareness of the pacing into the applications.
Adaptive applications, such as adaptive video streaming, are designed to deal with fluctuating goodput.
For the example of video streaming this adaption results in quality switches, reduced average quality and/or playback stalling events.
We argue that those adaptation algorithms could profit from being aware of the available goodput and less fluctuations.
Similar, other applications could fine-tune their network parameters, such as number of opened sockets, to adapt to the managed situation.

%\begin{itemize}
%\item Fail-safe possible: Switch back to TCP congestion control
%\item Additional parameters to evaluate: TCP algorithm, token bucket rate limiting, first hop pacing, etc.
%\end{itemize}
